End-to-end training of time domain audio separation and recognition

The rising interest in single-channel multi-speaker speech separation sparked development of End-to-End (E2E) approaches to multi-speaker speech recognition. However, up until now, state-of-the-art neural network-based time domain source separation has not yet been combined with E2E speech recognition. We here demonstrate how to combine a separation module based on a Convolutional Time domain Audio Separation Network (Conv-TasNet) with an E2E speech recognizer and how to train such a model jointly by distributing it over multiple GPUs or by approximating truncated back-propagation for the convolutional front-end. To put this work into perspective and illustrate the complexity of the design space, we provide a compact overview of single-channel multi-speaker recognition systems. Our experiments show a word error rate of 11.0% on WSJ0-2mix and indicate that our joint time domain model can yield substantial improvements over cascade DNN-HMM and monolithic E2E frequency domain systems proposed so far.

==> Makefile <==
SHELL=/bin/bash

main := main
target := ../arXiv

cmp:
	# Download the view.pdf from arXiv and verify that they are equal
	diffpdf ${main}.pdf view.pdf

clean:
	rm -rf ${target}

../arXiv:
	cp -r ../icassp2020_raw $@
	rm -rf $@/.git

	# cd $@ && rm Template.tex

	# https://arxiv.org/help/00README
	cd $@ && echo 'nohypertex' > 00README.XXX

	# Rarely nessesary
	# cd arXiv && echo 'convBF.tex toplevelfile' >> 00README.XXX

	# Force arXiv to use pdflatex
	# Prepend "\pdfoutput=1\n" to the main file
	cd $@ && sed -i '1s;^;\\pdfoutput=1\n;' ${main}.tex

	cd $@ && pdflatex -interaction=nonstopmode -shell-escape ${main}.tex > ../pdflatex_1.log
	cd $@ && bibtex ${main}
	cd $@ && pdflatex -interaction=nonstopmode -shell-escape ${main}.tex > ../pdflatex_2.log
	cd $@ && pdflatex -interaction=nonstopmode -shell-escape ${main}.tex > ../pdflatex_3.log

	# \includegraphics{PB2019.eps} produces error on arXiv
	# -> ! Package pdftex.def Error: File `PB2019.pdf' not found.
	#	 cd $@ && mv PB2019-eps-converted-to.pdf PB2019.pdf

	# cd $@ && rm $(main).{acn,acr,glg,glo,gls,bbl,alg}  # keep for arxiv
	cd $@ && rm ${main}.{aux,blg,log}
	# cd $@ && rm $(main).{ist,lof,lot,out,run.xml,toc}  # does not exist
	# cd $@ && rm $(main)-blx.bib  # does not exist

	# cd $@ && rm convBF.synctex.gz
	cd $@ && mv ${main}.pdf ..
	tar -czf $@.tar.gz -C $@ .



